Automatically Correcting Large Language Models: Surveying the landscape of diverse self-correction strategies

Large language models (LLMs) have demonstrated remarkable performance across a wide array of NLP tasks. However, their efficacy is undermined by undesired and inconsistent behaviors, including hallucination, unfaithful reasoning, and toxic content. A promising approach to rectify these flaws is self-correction, where the LLM itself is prompted or guided to fix problems in its own output. Techniques leveraging automated feedback -- either produced by the LLM itself or some external system -- are of particular interest as they are a promising way to make LLM-based solutions more practical and deployable with minimal human feedback. This paper presents a comprehensive review of this emerging class of techniques. We analyze and taxonomize a wide array of recent work utilizing these strategies, including training-time, generation-time, and post-hoc correction. We also summarize the major applications of this strategy and conclude by discussing future directions and challenges.

==> backup.tex <==
% a strategy that mirrors the human learning process where
% Feedback plays a crucial role in human learning. 
% When humans make mistakes, they often receive feedback, either from others or through self-reflection. This feedback provides insights into what went wrong and suggests potential areas for improvement. 
% Feedback can be explicit, like a teacher correcting a student's math problem, or implicit, such as a musician adjusting their technique based on the sound they produce. 
% From this feedback, humans can adapt and modify their behavior, learning to correct their mistakes over time. This capability to learn from feedback is a key component of human intelligence, contributing significantly to our ability to acquire new skills, improve performance, and solve complex problems. Motivated by this, significant research has been conducted on how to improve LLMs by learning from feedback. 

% Human learning is inherently iterative, with feedback playing a crucial role in this process. When humans make mistakes, they often receive feedback, either from others or through self-reflection, about the inaccuracies in their actions or decisions. This feedback mechanism is instrumental in human learning and growth. It serves as a mirror, providing insights into what went wrong and suggesting potential areas for improvement. Feedback can be explicit, like a teacher correcting a student's math problem, or implicit, such as a musician adjusting their technique based on the sound they produce. From this feedback, humans can adapt and modify their behavior, learning to correct their mistakes over time. This capability to learn from feedback is a key component of human intelligence, contributing significantly to our ability to acquire new skills, improve performance, and solve complex problems.



% Large language models have an impressive ability to "understand" and apply prompt instructions to generate or modify text. This has lead to a new design pattern where sophisticated classification, generation, editing, and retrieval modules in natural language systems are implemented purely using specialized prompts with an LLM. We dub this LLM-based module building approach "implementation \ourterm{}" and find that this enables insight in analyzing the explosion of self-correcting LLM-based approaches to a diverse array of tasks. We focus our analysis on an exciting subset of these approaches, where \ourterm self-correction is implemented, and model editing and correction capabilities are coordinated to improve performance and recover from prior failure cases. We analyze and taxonomize a wide array of recent work utilizing these approaches and discuss the fundamental LLM capabilities that make this "self-healing \ourterm{}" possible. With an understanding of the capabilities employed, we can shine a light on potential edge cases for improved robustness, and predict how future NLP capabilities will improve with as improved LLM capabilities lead to more sophisticated modules \ourterm.
%Lately, attempts to build robust and performant natural language generation systems have converged to an \textit{interactive} design pattern.
%In this paradigm, large language models are connected to external modules or separate language models, supervised by additional models, or prompted in such a way to self-refine and self-correct errors.
%We provide an overview of this novel set of recovery strategies and methodologies for systemic failure, capturing of world knowledge, incorporating existing knowledge bases, intrinsic evaluation, and discuss how it might influence future NLP research.

% "The idea of large language models being able to self-repair and self-fix used to be sci-fi"
% - we have only found a limited amount of knowledge and abilities in models so far through the SSL objective
% - collaboration between LLMs and non-LLMs
% - collaboration between different LLMs
% - self-play and self-repair to better make use of knowledge in the model
% - updating and repairing the models
% - training-free self-repair
% - a lot of benefits from getting a distribution out rather than point estimates, using a reward model to fix grammatical and syntax issues

% \begin{table*}[!t]
% \centering
% \resizebox{\textwidth}{!}{
%     \begin{tabular}% {c|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}|C{1.3cm}C{1.3cm}C{1.3cm}}
%     {lccccc}
%     \toprule
%         \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Critic}} & \multirow{2}{*}{\textbf{Feedback}} & \multicolumn{2}{c}{\textbf{Refiner}} & \multirow{2}{*}{\textbf{Application}} \\ 
%         & & & \textbf{Strategy} & \textbf{Learning} & \\ \midrule
%         CRITIC~\cite{Gou2023CRITICLL} & External Tools & NL & Post-hoc & ICL & \tabincell{c}{QA, Program Synthesis, \\ Toxicity Reduction} \\ \midrule
%         RARR~\cite{gao2023rarr} & External Knowledge & NL & Post-hoc & ICL & Reduce Hallucination \\ \midrule
%         \citet{olausson2023demystifying} & Program Executor & NL & Post-hoc & ICL & Code Generation \\
%         Self-Edit~\cite{zhang2023selfedit} & Program Executor & NL & Post-hoc & ICL & Code Generation \\
%         Self-Debug~\cite{chen2023teaching} & Program Executor & NL & Post-hoc & ICL & Code Generation \\
%         \bottomrule
%     \end{tabular}
% } 
%     \caption{Related works on verification and correction.}
%     \label{tbl:summary_works}
% \end{table*}




Because \ourterm implementations of many different capabilities require correct answers at output. As chain-of-thought (CoT) is considered to rely on a sequence of correct steps, \citet{xue2023rcot} consider using self-correction strategies to improve the factuality of intermediate CoT steps. From the logic that uses incorrect answers work well as a pseudolabel for incorrect CoTs, they leverage an \ourterm process to reconstruct original problem from reasoning chain and answer, which can then be compared to the original prompt \ourterm to ascertain whether further self-correction needs to be targeted. This ``reverse chain-of-thought'' (RCOT) leads to a 1-5\% gain in accuracy on an array of mathematical reasoning benchmarks.

\subsection{Prompt optimization}

\citet{zhou2022teaching} describe the technique of ``algorithmic prompting'' where the steps of simple arithmetic problems are described as detailed algorithms. For each in-context learning example, demonstrating an operation (eg. three-digit addition) numbers are split into pseudocode-like lists of digits and the steps involved are shown algorithmically using detailed natural language, which is found to be more performant on high-digit arithmetic problems than providing a simple scratchpad \cite{nye2021work, anil2022exploring} or chain of thought prompts \cite{wei2023chainofthought}. The performance of even a simple operation \ourterm such as arithmetic demonstrates considerable brittleness to prompting quality and strategy. 


\subsection{Feedback from external modules}

Many metrics and analysis paradigms are useful for targeting self-correcting interventions.
These metrics can work as external modules assessing a range of desired qualities for correction from faithfulness to \todo{correctness?}. 

\ms{This might need to move to a section about how ``demonstrating improvement is a challenge because we need metrics'' somewhere in 4 since this is an evaluation point not an in-the-loop point} Among faithfulness metrics, SARI \cite{xu2016optimizing}, originally developed for assessing machine translation, has been found to be well-correlated with human judgements of reference-based faithfulness and factuality in LM-generated answers to question answering datasets like FEVER and SciFact \cite{huang2023zeroshot}. 

\subsection{Verifier-guidance}

\subsection{Iterative approaches}

\subsection{Self-guidance}

The approach for RCOT \cite{xue2023rcot} fits in the self-guidance paradigm because the model is producing its own reversed question, based on which the decision for whether or not to execute further self-correction is made.

Similarly, ZeroFEC \cite{huang2023zeroshot} employs a process for the claim correction task where input (potentially unfaithful) claims are converted/decomposed into questions, answers to the questions are collected from a paired evidence passage, and the corresponding QA pairs are used to produce new, potentially corrected claims, all \ourterm{}.



==> full_table.tex <==
\begin{table*}[!t]
\centering
\resizebox{\textwidth}{!}{
   \begin{tabular}% 
   {lcccccc}
    \toprule
        \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Feedback}} & \multicolumn{3}{c}{\textbf{Model Refinement}} & \multirow{2}{*}{\textbf{Application}} \\ \cline{2-6}
        & \textbf{Source} & \textbf{Format} & \textbf{Strategy} & \textbf{Learning} & \textbf{Iter.} & \\ \midrule
        \rowcolor{LightCyan} \multicolumn{7}{c}{\textbf{Training-Time Correction}} \\ \midrule
        % RLHF
        RLHF~\cite{DBLP:conf/nips/Ouyang0JAWMZASR22} & Reward Model & Scalar & RLHF & RL & \usym{2717} & Multiple Tasks \\
        % Fine-grained RLHF
        Fine-Grained RLHF~\cite{wu2023finegrained} & Reward Model & Scalar & RLHF & RL & \usym{2717} & Detoxification, Long-form QA \\
        % HH-RLHF
        HH-RLHF~\cite{bai2022training} & Reward Model & Scalar & RLHF & SL \& RL & \usym{2713} & Helpfulness, Harmlessness \\
        % Moral Self-Correction
        % Moral RLHF~\cite{ganguli2023capacity} & Reward Model & Scalar & RLHF & RL & \usym{2717} & Moral Correction \\
        % Imitation learning from Language Feedback (ILF)
        % Sparrow
        Sparrow~\cite{glaese2022improving} & Reward Model & NL & RLHF & SL \& RL & \usym{2717} & Dialogue \\
        % ILF
        ILF~\cite{scheurer2023training} & Human Feedback & NL & Fine-tuning & SL & \usym{2713} & Summarization \\
        % Continually Improving Extractive QA via Human Feedback
        \citet{gao2023continually} & Human Feedback & NL & Fine-tuning & SL \& RL & \usym{2717} & Extractive QA \\
        % Chain-of-Hindsight
        Chain-of-Hindsight~\cite{liu2023chain} & Human Feedback & NL & Fine-tuning & SL & \usym{2717} & Multiple Tasks \\
        % Quark
        Quark~\cite{DBLP:conf/nips/LuWHJQWA022} & External Metrics & Scalar & Fine-tuning & RL & \usym{2717} &  Toxicity, Repetition, Sentiment \\
        % traditional method
        % Minimum Risk Training~\cite{shen-etal-2016-minimum} & External Metrics & Scalar & Fine-tuning & SL & \usym{2717} & Machine Translation \\
        % SimCLS
        SimCLS~\cite{liu-liu-2021-simcls} & External Metrics & Scalar & Fine-tuning & SL & \usym{2717} & Summarization \\
        % BERTTune
        BERTTune~\cite{unanue2021berttune} & External Metrics & Scalar & Fine-tuning & RL & \usym{2717} & Machine Translation \\
        % STaR
        STaR~\cite{zelikman2022star} & Language Model & NL & Self-Training & SL & \usym{2717} & QA, Reasoning \\
        % Self-Instruct
        Self-Instruct~\cite{DBLP:conf/acl/WangKMLSKH23} & Language Model & NL & Self-Training & SL & \usym{2717} & Multiple Tasks \\
        % Constitutional AI
        RLAIF~\cite{bai2022constitutional} & Language Model & NL & Self-Training & SL \& RL & \usym{2717} & Dialogue \\
        % SIRLC
        SIRLC~\cite{pang2023language} & Language Model & NL & Self-Training & RL & \usym{2717} & Reasoning, Trans., Summ. \\
        % Self-Improve
        Self-Improve~\cite{huang2022large} & Language Model & NL & Self-Training & SL & \usym{2717} & QA, Reasoning, NLI \\
        % AlpacaFarm
        AlpacaFarm~\cite{dubois2023alpacafarm} & Language Model & NL & Self-Training & SL \& RL & \usym{2717} & None (Intrinsic Evaluation) \\
        %%%%%%
        \midrule
        \rowcolor{LightCyan} \multicolumn{7}{c}{\textbf{Generation-Time Correction}} \\ 
        \midrule
        %%%%%%
        % Self-Verification
        Self-Verification~\cite{weng2023large} & Language Model & Scalar & Re-Ranking & ICL & \usym{2717} & Arithmetic Reasoning \\ 
        % CodeT
        CodeT~\cite{DBLP:conf/iclr/ChenZNZLLC23} & Program Executor & Scalar & Re-Ranking & ICL & \usym{2717} & Code Generation \\
        % LEVER
        LEVER~\cite{ni2023lever} & Program Executor & Scalar & Re-Ranking & SL & \usym{2717} & Table QA, Math QA, Program \\
        % Rethinking
        RR~\cite{he2022rethinking} & External Knowledge & Scalar & Re-Ranking & --- & \usym{2717} & Reasoning \\
        % InstructScore
        InstructScore~\cite{xu2023instructscore} & Language Model & NL & Re-Ranking & SL & \usym{2717} & Generation Evaluation \\
        % Minimum bayes risk decoding
        MBR Decoding~\cite{freitag-etal-2022-high} & External Metrics & Scalar & Re-Ranking & SL & \usym{2717} & Machine Translation \\
        % DIVERSE
        DIVERSE~\cite{li-etal-2023-making} & Trained Model & Scalar & Re-Ranking & SL & \usym{2717} & Arithmetic Reasoning \\
        % TeachMe
        % TeachMe~\cite{DBLP:conf/emnlp/MishraTC22} & Human Feedback & NL & Feedback-guided & SL & \usym{2717} & Proof Generation \\
        % Let's verify step-by-step
        PRM~\cite{lightman2023lets} & Reward Model & Scalar & Feedback-guided & SL & \usym{2717} & Arithmetic Reasoning \\
        % DiffusionLM
        DiffusionLM~\cite{Li-2022-DiffusionLM} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Controlled Text Generation \\
        % PPLM
        % PPLM~\cite{Dathathri2020Plug} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Controlled Text Generation \\
        % Fudge
        Fudge~\cite{yang-klein-2021-fudge} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Controlled Text Generation \\
        % Entailer
        Entailer~\cite{DBLP:conf/emnlp/TafjordMC22} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Proof Generation \\
        % NLProofS
        NLProofS~\cite{DBLP:conf/emnlp/Yang0C22} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Proof Generation \\
        % GRACE
        GRACE~\cite{KhalifaGRACE} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Arithmetic Reasoning \\
        % CoRe
        CoRe~\cite{DBLP:conf/acl/ZhuWZZ0GZY23} & Trained Model & Scalar & Feedback-guided & SL & \usym{2717} & Arithmetic Reasoning \\
        % Maieutic Prompting
        Maieutic Prompting~\cite{DBLP:conf/emnlp/JungQWBB0C22} & External Metrics & Scalar & Feedback-guided & ICL & \usym{2717} & Commonsense Reasoning \\
        % Selection-Inference
        SI~\cite{DBLP:SelectionInference} & Language Model & Scalar & Feedback-guided & ICL & \usym{2717} & Proof Generation \\
        % RAP
        RAP~\cite{hao2023reasoning} & Language Model & Scalar & Feedback-guided & ICL & \usym{2717} & Planning, Reasoning \\
        % Self-Evaluation Guided Decoding
        SelfEval-Decoding~\cite{xie2023decomposition} & Language Model & Scalar & Feedback-guided & ICL & \usym{2717} & Arithmetic / Symbolic Reasoning \\
        % Tree-of-Thought
        Tree of Thoughts~\cite{yao2023tree} & Language Model & NL / Scalar & Feedback-guided & ICL & \usym{2717} & Games, Writing \\
        %%%%%%
        \midrule
        \rowcolor{LightCyan} \multicolumn{7}{c}{\textbf{Post-hoc Correction}} \\ 
        \midrule
        %%%%%%
        % Self-Refine
        Self-Refine~\cite{madaan2023selfrefine} & Language Model & NL & Self-Refine & ICL & \usym{2713} & Multiple Tasks \\
        % PEER
        % PEER~\cite{schick2022peer} & Language Model & NL & Post-hoc & SL & \usym{2713} & Text Editing \\
        % Clinical information extraction
        Clinical SV~\cite{gero2023selfverification} & Language Model & NL & Self-Refine & ICL & \usym{2717} & Information Extraction \\
        % Reflexion
        % \tabincell{c}{Decision-making, QA, \\ Code Generation}
        Reflexion~\cite{shinn2023reflexion} & Language Model & NL & Self-Refine & RL & \usym{2713} & QA, Code Generation \\
        % Iterative Improvement
        IterRefinement~\cite{Chen2023IterativeTR} & Language Model & NL & Self-Refine & ICL & \usym{2713} & Machine Translation \\
        % Auto-Post-Editing
        Auto-Post-Editing~\cite{raunak2023leveraging}  & Language Model & NL & Self-Refine & ICL & \usym{2717} & Machine Translation \\
        % RCI
        RCI~\cite{kim2023language} & Language Model & NL & Self-Refine & ICL & \usym{2713} & Computer Tasks \\
        % Selfee
        SelFee~\cite{selfee2023} & Language Model & NL & Self-Refine & SL & \usym{2713} & Dialogue \\
        % SelfCheckGPT
        SelfCheckGPT~\cite{manakul2023selfcheckgpt} & Language Model & NL & Self-Refine & ICL & \usym{2717} & Hallucination Detection \\
        % Re3
        Re$^3$~\cite{yang-etal-2022-re3} & Trained Model & Scalar & External Feedback & SL \& ICL & \usym{2713} & Story Generation \\
        % CodeRL
        CodeRL~\cite{le2022coderl} & Trained Model & Scalar & External Feedback & RL & \usym{2717} & Code Generation \\
        % REFINER
        REFINER~\cite{paul2023refiner} & Trained Model & NL & External Feedback & SL \& ICL & \usym{2713} & Reasoning, Moral Story \\
        % RL4F
        RL4F~\cite{DBLP:conf/acl/AkyurekAKCWT23} & Trained Model & NL & External Feedback & SL \& RL & \usym{2713} & Planning, Summarization \\
        % Feedback for Interactive Semantic Parsing
        \citet{DBLP:conf/acl/YanSTWYY23} & Trained Model & NL & External Feedback & SL & \usym{2713} & Semantic Parsing \\
        % Baldur
        Baldur~\cite{first2023baldur} & Trained Model & NL & External Feedback & ICL & \usym{2713} & Proof Generation \\
        % CRITIC
        CRITIC~\cite{Gou2023CRITICLL} & External Tools & NL & External Feedback & ICL & \usym{2713} & QA, Program, Toxicity \\ 
        % FacTool
        FacTool~\cite{chern2023factool} & External Tools & NL & External Feedback & ICL & \usym{2713} & QA, Reasoning, Generation \\
        % RARR
        RARR~\cite{gao2023rarr} & External Knowledge & NL & External Feedback & ICL & \usym{2717} & Open-Domain QA \\ 
        % LLM-Augmenter
        LLM-Augmenter~\cite{peng2023check} & External Knowledge & NL & External Feedback & RL & \usym{2713} & Open-Domain QA \\
        % Self-Checker
        Self-Checker~\cite{li2023selfchecker} & External Knowledge & NL & External Feedback & ICL & \usym{2717} & Fact-Checking \\
        % REFEED
        REFEED~\cite{yu2023improving} & External Knowledge & NL & External Feedback & ICL & \usym{2717} & QA, Dialogue \\ 
        % Demystifying
        \citet{olausson2023demystifying} & Program Executor & NL & External Feedback & ICL & \usym{2713} & Code Generation \\
        % Self-Edit
        Self-Edit~\cite{zhang2023selfedit} & Program Executor & NL & External Feedback & ICL & \usym{2713} & Code Generation \\
        % Self-debug
        Self-Debug~\cite{chen2023teaching} & Program Executor & NL & External Feedback & ICL & \usym{2713} & Code Generation \\
        % Self-Evolve
        Self-Evolve~\cite{jiang2023selfevolve} & Program Executor & NL & External Feedback & ICL & \usym{2713} & Code Generation \\
        % Logic-LM
        Logic-LM~\cite{pan2023logiclm} & Symbolic Solver & NL & External Feedback & ICL & \usym{2713} & Logical Reasoning \\
        % Self-Critique
        Self-Critique~\cite{Saunders2022SelfcritiquingMF} & LLMs + Human & NL & External Feedback & SL & \usym{2717} & Summarization \\
        % ALGO
        ALGO~\cite{zhang2023algo} & Oracle Verifier & Scalar & External Feedback & ICL & \usym{2713} & Code Generation \\
        % Self-Healing Software
        \citet{charalambous2023new} & Bounded Model Checker & NL & External Feedback & ICL & \usym{2717} & Software Verification \\
        % Self-Correct
        Self-Correction~\cite{DBLP:conf/iclr/WelleckLWBSK023} & External Metrics & NL / Scalar & External Feedback & SL & \usym{2713} & Reasoning, Generation, Toxicity \\
        % Multiagent Debate
        Multiagent Debate~\cite{du2023improving} & Language Model & NL & Model Debate & ICL & \usym{2713} & Reasoning, Factuality \\
        % LM vs LM
        LM vs LM~\cite{cohen2023lm} & Language Model & NL & Model Debate & ICL & \usym{2713} & Factual Error Detection \\
        % ICL-AIF
        ICL-AIF~\cite{fu2023improving} & Language Model & NL & Model Debate & ICL & \usym{2713} & Bargaining Game \\
        % PRD
        PRD~\cite{li2023prd} & Language Model & NL & Model Debate & ICL & \usym{2713} & Open-ended QA \\
        \bottomrule
   \end{tabular}
} 
    \caption{A summary of representative works on correcting large language models with automated feedback. % The methods are organized into three major categories based on the criteria introduced in Section~\ref{subsec:when_feedback}: \textit{Training-Time}, \textit{Generation-Time}, and \textit{Post-hoc Correction}. 
    We summarize the key features for each work: the \textbf{source} and \textbf{format} of the feedback, the \textbf{strategy} and \textbf{learning} method of the refinement process, whether the refinement is iterative \textbf{(Iter.)}, and the \textbf{application} of the method.}
    \label{tbl:summary_works}
\end{table*}
